Gamma Related Ornstein-Uhlenbeck Processes and their Simulation

We investigate the distributional properties of two generalized Ornstein-Uhlenbeck (OU) processes whose stationary distributions are the gamma law and the bilateral gamma law, respectively. The said distributions turn out to be related to the self-decomposable gamma and bilateral gamma laws, and their densities and characteristic functions are here given in closed-form. Algorithms for the exact generation of such processes are accordingly derived with the advantage of being significantly faster than those available in the literature and therefore suitable for real-time simulations.

==> Tables/TableGasStorageSpec.tex <==
\begin{table}
    \centering
    \begin{tabular}{|c|c|c|c|c|}
            \hline
             $C(0) $   &  $C(T) $ & $a_{in} $  & $a_{w}$ & $C_{max} $ \\
          \hline
             0  &  0 &  $1$ &  $1$ &  $20$ \\	
	    \hline
    \end{tabular}
    \small
    \caption{Fast Storage Specification.}\label{tab:storage:spec}
\end{table}


==> Tables/TableGasSwingSpec.tex <==
\begin{table}
    \centering
    \begin{tabular}{|c|c|c|c|c|}
            \hline
             $ACQmin$   &  $ACQmax$ & $DCQmin$  & $DCQmax$ & $T (days)$ \\
          \hline
             120  &  120 &  $1$ &  $1$ &  $360$ \\	
	    \hline
    \end{tabular}
    \small
    \caption{Specification of 120-120 take-or-pay Swing}\label{tab:swing:spec}
\end{table}


==> Tables/TableMoments.tex <==
%\begin{table}
    %\centering
    %\subtable{
        %\begin{tabular}{|c|c|c|c|c|c|c|}
          %\hline
           %after \\: \hline or \cline{col1-col2} \cline{col3-col4} ...
            %$\lambda_P$ & $\lambda_J$ & $k$ & $\alpha$ & $\Delta t_m$ & $a$ & $N$\\
            %\hline
            %10 & 1& 36 & 0.2778 & 1/365 & 0.9061 & $40$\\
          %\hline
        %\end{tabular}
        %}
    %\small
    %\caption{Parameters used in the MC simulation in Table \myref{tab:Moments:MC} with $10^6$ scenarios}\label{tab:Parameters:MC}
%\end{table}
\begin{table}
    \centering
%    \subtable{
        \begin{tabular}{|c|c|c|c|c|}
          \hline
          % after \\: \hline or \cline{col1-col2} \cline{col3-col4} ...
            Order & Exact & Algorithm 1 & Algorithm 2 & Algorithm 4\\
            \hline
            1 &$0.0261$ &$0.0260$ &$0.0262$ & $0.0261$ \\
            \hline
            2 &$0.0504$ &$0.0501$ &$0.0503$& $0.0569$ \\
            \hline
            3 &$0.1462$ &$0.1437$ &$0.1428$& $0.1434$ \\
            \hline
            4 &$0.5658$ &$0.5433$ & $0.5719$ & $0.5351$\\
            \hline
            5 &$2.7389$ &$2.5223$ &$2.8930$& $2.4177$\\
            \hline
        \end{tabular}
 %   }
    \small
    \caption{Moments calculated with Algorithms \myref{alg:sd} and\myref{alg:sd:gamma},\myref{alg1:ref}, }\label{tab:Moments:MC}
\end{table}






